Near-optimal matrix recovery from random linear measurements

In matrix recovery from random linear measurements, one is interested in recovering an unknown $M$-by-$N$ matrix $X_0$ from $n<MN$ measurements $y_i=Tr(A_i^T X_0)$ where each $A_i$ is an $M$-by-$N$ measurement matrix with i.i.d random entries, $i=1,\ldots,n$. We present a novel matrix recovery algorithm, based on approximate message passing, which iteratively applies an optimal singular value shrinker -- a nonconvex nonlinearity tailored specifically for matrix estimation. Our algorithm typically converges exponentially fast, offering a significant speedup over previously suggested matrix recovery algorithms, such as iterative solvers for Nuclear Norm Minimization (NNM). It is well known that there is a recovery tradeoff between the information content of the object $X_0$ to be recovered (specifically, its matrix rank $r$) and the number of linear measurements $n$ from which recovery is to be attempted. The precise tradeoff between $r$ and $n$, beyond which recovery by a given algorithm becomes possible, traces the so-called phase transition curve of that algorithm in the $(r,n)$ plane. The phase transition curve of our algorithm is noticeably better than that of NNM. Interestingly, it is close to the information-theoretic lower bound for the minimal number of measurements needed for matrix recovery, making it not only state-of-the-art in terms of convergence rate, but also near-optimal in terms of the matrices it successfully recovers.

==> figures/PTPlots/PTPlot_Dump.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{PTPlots/PTCurve_N=100_beta=0.5_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=100$, $\beta=0.5$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{PTPlots/PTCurve_N=100_beta=1.0_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=100$, $\beta=1.0$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{PTPlots/PTCurve_N=50_beta=0.2_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=50$, $\beta=0.2$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{PTPlots/PTCurve_N=50_beta=0.4_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=50$, $\beta=0.4$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{PTPlots/PTCurve_N=50_beta=0.6_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=50$, $\beta=0.6$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{PTPlots/PTCurve_N=50_beta=0.8_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=50$, $\beta=0.8$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{PTPlots/PTCurve_N=50_beta=1.0_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=50$, $\beta=1.0$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{PTPlots/PTCurve_N=100_beta=0.2_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=100$, $\beta=0.2$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{PTPlots/PTCurve_N=100_beta=0.4_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=100$, $\beta=0.4$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{PTPlots/PTCurve_N=100_beta=0.6_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=100$, $\beta=0.6$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{PTPlots/PTCurve_N=100_beta=0.8_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=100$, $\beta=0.8$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{PTPlots/PTCurve_N=100_beta=1.0_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=100$, $\beta=1.0$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{PTPlots/PTCurve_N=150_beta=0.2_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=150$, $\beta=0.2$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{PTPlots/PTCurve_N=150_beta=0.4_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=150$, $\beta=0.4$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{PTPlots/PTCurve_N=150_beta=0.6_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=150$, $\beta=0.6$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{PTPlots/PTCurve_N=150_beta=0.8_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=150$, $\beta=0.8$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{PTPlots/PTCurve_N=150_beta=1.0_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=150$, $\beta=1.0$, required precision=$0.001$.}
\end{figure}


==> figures/Rates/rates_figs.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=3.0in]{figures/{Rates/figRates_N=50_beta=1.0_rho=0.04_delta_diff=0.03}.pdf}
    \caption{Convergence rate above the PT: 
    $N=50$, $\beta=1.0$, $\rho=0.04$, $\delta=\delta^*$+0.03}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=3.0in]{figures/{Rates/figRates_N=50_beta=1.0_rho=0.04_delta_diff=0.1}.pdf}
    \caption{Convergence rate above the PT: 
    $N=50$, $\beta=1.0$, $\rho=0.04$, $\delta=\delta^*$+0.1}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=3.0in]{figures/{Rates/figRates_N=50_beta=1.0_rho=0.1_delta_diff=0.03}.pdf}
    \caption{Convergence rate above the PT: 
    $N=50$, $\beta=1.0$, $\rho=0.1$, $\delta=\delta^*$+0.03}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=3.0in]{figures/{Rates/figRates_N=50_beta=1.0_rho=0.1_delta_diff=0.1}.pdf}
    \caption{Convergence rate above the PT: 
    $N=50$, $\beta=1.0$, $\rho=0.1$, $\delta=\delta^*$+0.1}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=3.0in]{figures/{Rates/figRates_N=50_beta=1.0_rho=0.2_delta_diff=0.03}.pdf}
    \caption{Convergence rate above the PT: 
    $N=50$, $\beta=1.0$, $\rho=0.2$, $\delta=\delta^*$+0.03}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=3.0in]{figures/{Rates/figRates_N=50_beta=1.0_rho=0.2_delta_diff=0.1}.pdf}
    \caption{Convergence rate above the PT: 
    $N=50$, $\beta=1.0$, $\rho=0.2$, $\delta=\delta^*$+0.1}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=3.0in]{figures/{Rates/figRates_N=50_beta=1.0_rho=0.4_delta_diff=0.03}.pdf}
    \caption{Convergence rate above the PT: 
    $N=50$, $\beta=1.0$, $\rho=0.4$, $\delta=\delta^*$+0.03}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=3.0in]{figures/{Rates/figRates_N=50_beta=1.0_rho=0.4_delta_diff=0.1}.pdf}
    \caption{Convergence rate above the PT: 
    $N=50$, $\beta=1.0$, $\rho=0.4$, $\delta=\delta^*$+0.1}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=3.0in]{figures/{Rates/figRates_N=100_beta=0.5_rho=0.04_delta_diff=0.03}.pdf}
    \caption{Convergence rate above the PT: 
    $N=100$, $\beta=0.5$, $\rho=0.04$, $\delta=\delta^*$+0.03}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=3.0in]{figures/{Rates/figRates_N=100_beta=0.5_rho=0.04_delta_diff=0.1}.pdf}
    \caption{Convergence rate above the PT: 
    $N=100$, $\beta=0.5$, $\rho=0.04$, $\delta=\delta^*$+0.1}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=3.0in]{figures/{Rates/figRates_N=100_beta=0.5_rho=0.1_delta_diff=0.03}.pdf}
    \caption{Convergence rate above the PT: 
    $N=100$, $\beta=0.5$, $\rho=0.1$, $\delta=\delta^*$+0.03}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=3.0in]{figures/{Rates/figRates_N=100_beta=0.5_rho=0.1_delta_diff=0.1}.pdf}
    \caption{Convergence rate above the PT: 
    $N=100$, $\beta=0.5$, $\rho=0.1$, $\delta=\delta^*$+0.1}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=3.0in]{figures/{Rates/figRates_N=100_beta=0.5_rho=0.2_delta_diff=0.03}.pdf}
    \caption{Convergence rate above the PT: 
    $N=100$, $\beta=0.5$, $\rho=0.2$, $\delta=\delta^*$+0.03}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=3.0in]{figures/{Rates/figRates_N=100_beta=0.5_rho=0.2_delta_diff=0.1}.pdf}
    \caption{Convergence rate above the PT: 
    $N=100$, $\beta=0.5$, $\rho=0.2$, $\delta=\delta^*$+0.1}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=3.0in]{figures/{Rates/figRates_N=100_beta=0.5_rho=0.4_delta_diff=0.03}.pdf}
    \caption{Convergence rate above the PT: 
    $N=100$, $\beta=0.5$, $\rho=0.4$, $\delta=\delta^*$+0.03}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=3.0in]{figures/{Rates/figRates_N=100_beta=0.5_rho=0.4_delta_diff=0.1}.pdf}
    \caption{Convergence rate above the PT: 
    $N=100$, $\beta=0.5$, $\rho=0.4$, $\delta=\delta^*$+0.1}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=3.0in]{figures/{Rates/figRates_N=100_beta=1.0_rho=0.04_delta_diff=0.03}.pdf}
    \caption{Convergence rate above the PT: 
    $N=100$, $\beta=1.0$, $\rho=0.04$, $\delta=\delta^*$+0.03}
\end{figure}


==> figures/dump_pt_plots/PTPlot_Dump.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{dump_pt_plots/PTCurve_N=50_beta=0.2_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=50$, $\beta=0.2$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{dump_pt_plots/PTCurve_N=50_beta=0.4_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=50$, $\beta=0.4$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{dump_pt_plots/PTCurve_N=50_beta=0.6_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=50$, $\beta=0.6$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{dump_pt_plots/PTCurve_N=50_beta=0.8_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=50$, $\beta=0.8$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{dump_pt_plots/PTCurve_N=50_beta=1.0_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=50$, $\beta=1.0$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{dump_pt_plots/PTCurve_N=100_beta=0.2_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=100$, $\beta=0.2$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{dump_pt_plots/PTCurve_N=100_beta=0.4_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=100$, $\beta=0.4$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{dump_pt_plots/PTCurve_N=100_beta=0.6_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=100$, $\beta=0.6$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{dump_pt_plots/PTCurve_N=100_beta=0.8_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=100$, $\beta=0.8$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{dump_pt_plots/PTCurve_N=100_beta=1.0_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=100$, $\beta=1.0$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{dump_pt_plots/PTCurve_N=150_beta=0.2_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=150$, $\beta=0.2$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{dump_pt_plots/PTCurve_N=150_beta=0.4_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=150$, $\beta=0.4$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{dump_pt_plots/PTCurve_N=150_beta=0.6_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=150$, $\beta=0.6$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{dump_pt_plots/PTCurve_N=150_beta=0.8_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=150$, $\beta=0.8$, required precision=$0.001$.}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{dump_pt_plots/PTCurve_N=150_beta=1.0_tol=0.001}.pdf}
	\caption{Empirical PT curve: $N=150$, $\beta=1.0$, required precision=$0.001$.}
\end{figure}


==> figures/universality/universality_plots.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{universality/universality_denoiser=SPIKED_MMX_N=100_beta=0.5_rho=0.1}.pdf}
	\caption{Empirical success probability for different measurement matrix ensembles.
	Algorithm = \AMPOPT. $N=100$, $\beta=0.5$, $\rho=0.1$. }
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{universality/universality_denoiser=SVST_N=100_beta=0.5_rho=0.1}.pdf}
	\caption{Empirical success probability for different measurement matrix ensembles.
	Algorithm = \AMPSVST. $N=100$, $\beta=0.5$, $\rho=0.1$. }
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{universality/universality_denoiser=SPIKED_MMX_N=100_beta=0.5_rho=0.3}.pdf}
	\caption{Empirical success probability for different measurement matrix ensembles.
	Algorithm = \AMPOPT. $N=100$, $\beta=0.5$, $\rho=0.3$. }
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{universality/universality_denoiser=SPIKED_MMX_N=100_beta=0.5_rho=0.1}.pdf}
	\caption{Empirical success probability for different measurement matrix ensembles.
	Algorithm = \AMPOPT. $N=100$, $\beta=0.5$, $\rho=0.1$. }
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{universality/universality_denoiser=SVST_N=100_beta=0.5_rho=0.1}.pdf}
	\caption{Empirical success probability for different measurement matrix ensembles.
	Algorithm = \AMPSVST. $N=100$, $\beta=0.5$, $\rho=0.1$. }
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{universality/universality_denoiser=SPIKED_MMX_N=100_beta=0.5_rho=0.3}.pdf}
	\caption{Empirical success probability for different measurement matrix ensembles.
	Algorithm = \AMPOPT. $N=100$, $\beta=0.5$, $\rho=0.3$. }
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{universality/universality_denoiser=SVST_N=100_beta=0.5_rho=0.3}.pdf}
	\caption{Empirical success probability for different measurement matrix ensembles.
	Algorithm = \AMPSVST. $N=100$, $\beta=0.5$, $\rho=0.3$. }
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{universality/universality_denoiser=SPIKED_MMX_N=100_beta=1_rho=0.1}.pdf}
	\caption{Empirical success probability for different measurement matrix ensembles.
	Algorithm = \AMPOPT. $N=100$, $\beta=1$, $\rho=0.1$. }
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{universality/universality_denoiser=SVST_N=100_beta=1_rho=0.1}.pdf}
	\caption{Empirical success probability for different measurement matrix ensembles.
	Algorithm = \AMPSVST. $N=100$, $\beta=1$, $\rho=0.1$. }
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{universality/universality_denoiser=SPIKED_MMX_N=100_beta=1_rho=0.3}.pdf}
	\caption{Empirical success probability for different measurement matrix ensembles.
	Algorithm = \AMPOPT. $N=100$, $\beta=1$, $\rho=0.3$. }
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=3.0in]{figures/{universality/universality_denoiser=SVST_N=100_beta=1_rho=0.3}.pdf}
	\caption{Empirical success probability for different measurement matrix ensembles.
	Algorithm = \AMPSVST. $N=100$, $\beta=1$, $\rho=0.3$. }
\end{figure}

